Adaptive Natural Language Generation for Task-oriented Dialogue via Reinforcement Learning

When a natural language generation (NLG) component is implemented in a real-world task-oriented dialogue system, it is necessary to generate not only natural utterances as learned on training data but also utterances adapted to the dialogue environment (e.g., noise from environmental sounds) and the user (e.g., users with low levels of understanding ability). Inspired by recent advances in reinforcement learning (RL) for language generation tasks, we propose ANTOR, a method for Adaptive Natural language generation for Task-Oriented dialogue via Reinforcement learning. In ANTOR, a natural language understanding (NLU) module, which corresponds to the user's understanding of system utterances, is incorporated into the objective function of RL. If the NLG's intentions are correctly conveyed to the NLU, which understands a system's utterances, the NLG is given a positive reward. We conducted experiments on the MultiWOZ dataset, and we confirmed that ANTOR could generate adaptive utterances against speech recognition errors and the different vocabulary levels of users.

==> old_table.tex <==


\begin{table*}[t]
% \small
\centering
\begin{tabular}{ll|ccc|ccc|ccc|ccc} \bhline{0.8pt}
\ml{2}{l}{\mr{2}{{\bf Model}}}& \ml{12}{|c}{\textbf{SNR for background noise}} \\ \cline{3-14}
            &           & \ml{3}{|c|}{0}        & \ml{3}{c|}{5}         & \ml{3}{c|}{10}  & \ml{3}{c}{20}   \\ \cline{3-14}
NLG         & NLU       & Acc.  & F1    & WER   & Acc.  & F1    & WER   & Acc.  & F1    & WER   & Acc.  & F1    & WER   \\ \hline
SC-LSTM     & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  \\
SC-GPT      & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  \\ \hline
GPT-2       & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\
GPT-2-RL    & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\ \hline
SC-LSTM     & BERT      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\
SC-GPT      & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\ \hline
GPT-2       & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\
GPT-2-RL    & MILU      & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.*  & **.* \\ \bhline{0.8pt}
\end{tabular}
\caption{Scores for each NLG model when evaluated using MILU and BERT, trained using only the vocabulary lists defined at each level of the CEFR-J.}
\tbllabel{lower_vocab_env_result}
\end{table*}

\begin{table*}[t]
\small
\centering
\begin{tabular}{ll|cc|cc|cc|cc} \bhline{0.8pt}
\ml{2}{l}{\mr{2}{{\bf Model}}}& \ml{8}{|c}{\textbf{CEFR-J level}} \\ \cline{3-10}
            &           & \ml{2}{|c|}{$\leq$A1}  & \ml{2}{c|}{$\leq$A2}  & \ml{2}{c|}{$\leq$B1}  & \ml{2}{c}{$\leq$B2}  \\ \cline{3-10}
NLG         & NLU       & Acc.      & F1        & Acc.      & F1        & Acc.      & F1        & Acc.      & F1        \\ \hline
SC-LSTM     & MILU      & 47.4      & 53.9      & 55.7      & 62.5      & 62.4      & 68.8      & 63.6      & 69.8      \\
SC-GPT      & MILU      & 47.2      & 53.9      & 56.4      & 63.5      & 63.4      & 70.1      & 66.1      & 72.5      \\
GPT-2       & MILU      & 48.4      & 55.0      & 57.7      & 64.7      & 66.0      & 72.6      & 68.6      & 74.8      \\
GPT-2-RL    & MILU      & {\bf 54.7}      & {\bf 61.1}      & {\bf 63.5}      & {\bf 69.8}      & {\bf 72.5}      & {\bf 78.0}      & {\bf 75.0}      & {\bf 80.1}      \\ \hline
SC-LSTM     & BERT      & 68.6      & 73.6      & 72.0      & 76.3      & 72.8      & 76.9      & 73.1      & 77.2      \\
SC-GPT      & BERT      & 70.3      & 75.9      & 73.3      & 77.9      & 77.3      & 81.4      & 77.6      & 81.9      \\
GPT-2       & BERT      & 65.3      & 70.8      & 74.9      & 79.4      & 79.1      & 83.5      & 78.2      & 82.5      \\
GPT-2-RL    & BERT      & {\bf 83.0}      & {\bf 87.0}      & {\bf 85.7}      & {\bf 89.2}      & {\bf 87.8}      & {\bf 90.6}      & {\bf 87.7}      & {\bf 90.6}      \\ \bhline{0.8pt}
\end{tabular}
\caption{Scores for each NLG model when evaluated using MILU and BERT, trained using only the vocabulary lists defined at each level of the CEFR-J.}
\tbllabel{lower_vocab_env_result}
\end{table*}
